Leveraging Foundation Models to Improve Lightweight Clients in Federated Learning

Federated Learning (FL) is a distributed training paradigm that enables clients scattered across the world to cooperatively learn a global model without divulging confidential data. However, FL faces a significant challenge in the form of heterogeneous data distributions among clients, which leads to a reduction in performance and robustness. A recent approach to mitigating the impact of heterogeneous data distributions is through the use of foundation models, which offer better performance at the cost of larger computational overheads and slower inference speeds. We introduce foundation model distillation to assist in the federated training of lightweight client models and increase their performance under heterogeneous data settings while keeping inference costs low. Our results show improvement in the global model performance on a balanced testing set, which contains rarely observed samples, even under extreme non-IID client data distributions. We conduct a thorough evaluation of our framework with different foundation model backbones on CIFAR10, with varying degrees of heterogeneous data distributions ranging from class-specific data partitions across clients to dirichlet data sampling, parameterized by values between 0.01 and 1.0.

==> tex/intro.tex <==
\section{Introduction}
\label{sec:introduction}
% FL: what is FL
Federated learning (FL) is a decentralized training paradigm in machine learning~\cite{mcmahan2017communication} that addresses training one global model across multiple clients while preserving the privacy of locally-stored client data.
A typical FL framework consists of a central server that coordinates the global model's training by periodically aggregating local models collected from distributed clients, with each client's model trained with locally stored data.
% Core problems in FL: heterogeous data + communication / inference budget
As with many other distributed learning approaches, one of the major challenges for FL is that locally-stored client data are heterogeneous, which can be caused from uneven distribution or unbalanced patterns \cite{li2020federated1} and results in client-drift, commonly-seen accuracy drops, and non-convergence \cite{zhao2018federated, karimireddy2020scaffold, hsieh2020non, li2020federated1}. In addition, due to practical deployment in real-world contexts that clients impose strict limitations on inference speeds and communications bandwidth, it in turn restricts clients to use small-scale models. This poses an additional challenge to train a high-performing but lightweight global model.


% Foundation Models: A Potential Solution. WHY
In order to maintain satisfying performance under heterogeneous data distributions, foundation models~\cite{bommasani2021opportunities} present a potential solution to addressing poor performance. This is because one widely known benefit of foundation models are their comprehensive knowledge and transferable representations across a broad range of downstream tasks~\cite{radford2021learning,wang2022image}, and strong robustness to distribution shifts~\cite{ma2021simple}. Multiple recent methods explore fine-tuning transformer-based architectures and foundation models under federated settings \cite{qu2022rethinking, chen2022importance, guo2023promptfl, chen2022fedtune, su2022cross, guo2023pfedprompt}.
% Roadblocks 
There are lines of work trying to leverage foundation models under the setting of federated learning, {\color{red}\cite{chen2022fedtune} ...}. 
However, \cite{chen2022fedtune} have shown that under extreme non-IID conditions, federated training of foundation models forces a performance worse than purely local training. 
In addition, these methods do not discuss the relatively large increase in inference time when switching to foundation models instead of small-scale alternatives like EfficientNet~\cite{tan2019efficientnet}, MobileNet~\cite{sandler2018mobilenetv2}, etc.
% gap
% Therefore, there is definitely a gap in leveraging foundation models effectively to provide transferable knowledge to clients in a federated learning system, under the settings of non-iid data and the small-scale backbone training. 

% what we want to address
In order to leverage foundation models effectively to provide transferable knowledge under non-iid data as well as small-scale backbone training settings, we propose an approach to train lightweight proxy models in a federated manner under the supervision from foundation models. The proxy models to train and communicate in the federated learning system could offer model privacy on the foundation models that clients are referring to, because sometimes the information of foundation models being used to supervise local training is also a secrete in many global commercial parties and international companies. {\color{red}\st{On the other hand, as most federated training algorithms assume the exchange of a complete set or partial subset of weights with the server, it does not comply with the privacy constraint. More specifically, it has been previously shown that by capturing gradient updates or weights, a malicious user can infer multiple properties of the original data distribution and in turn use this information in an adversarial manner. Thus, a more protected training approach is in demand due to such privacy concerns. % ~\cite{melis2019exploiting,geiping2020inverting}
}}
{\color{blue}Add paragraph to show motivations and reason for our setup: 1. Why and in what applications do we need the more efficient proxy model 2. Why improving inference time is important in applications. }

% Our solution
Keeping in mind the considerations of heterogeneous data distributions, inference speed, and privacy, we propose a novel federated training framework that improves the overall performance of a lightweight model by distilling information from locally stored foundation models in clients.
% Performance under non-IID and privacy benefits
Our framework allows clients flexibility in the number and type of foundation models stored within each client, which allows the small-scale model to reap the benefits of improved performance as well as robustness to non-IID distributions and privacy-based optimization schemes, both of which are known to decrease overall performance.
% Size and speed benefits
In addition, our framework removes the computational burden of running a large foundation model during inference time by relying on the small-scale model to measure the overall performance of the client.
By treating the foundation model as a local model, the small-scale model as a proxy that can be shared. This reduce the communication cost and address the data privacy concerns as the system is training with privacy guaranteed optimization techniques \cite{abadi2016deep,esipova2022disparate}.

Overall our main contributions are as follows: 
\begin{itemize}
    % FMFL + small backbone training (distillation)
    % \item To the best of our knowledge, we are the first to leverage foundation models in federated learning settings under a restricted computational, communication and inference time budget. Our federated training framework increases the upper limit in performance and robustness achievable in small-scale client models. 
    \item This is the first approach to leverage foundation models in federated learning settings under a restricted computational, communication and inference time budget. This federated training framework increases the upper-limit in performance and robustness achievable in small-scale client models (\emph{e.g.} increase of {\color{red}$x_1\%$} for EfficientNet~\cite{tan2019efficientnet}, and increase of {\color{red}$x_2\%$} for MobileNet~\cite{sandler2018mobilenetv2}).

    % non-iid setting
    %\item Our work is robust to various and even strict level of data heterogeneity. Our thorough experiments show that our approach remains stable and high performances under different settings, which allows the system less sensitive to varying heterogeneous setting widely seen in practice.
    \item Our work robustly outperforms {\color{red}competing methods: FedAvg, FedProx, ProxyFL, with at least $\%$ accuracy increase} in a varying range of data heterogeneity, (from i.i.d to Dirichlet distribution with $\alpha=1$ to $0.01$ and class split), with lower performance decay in stricter data heterogeneity settings. Our experimental results show that our approach remains stable and achieves high performance under different data heterogeneity settings, allowing the system to be more robust in practice.

    
   
    % \item By distilling knowledge from foundation models, we overcome the drop in overall performance observed. We when using dp-SGD {\color{red}cite}, an optimization scheme with privacy guarantees.
     % model privacy and data security
    % Proxy model -> model privacy
    % dp-SGD -> data security
    % we boost accuracy, because we distill knowledge from foundation models
    \item {\color{red}\st{By combining a model-privacy approach (federated proxy models distilled from foundation models) with a data-security approach (an optimization approach with privacy guarantees - \emph{i.e.} dp-SGD {\color{red}cite}), we achieve an improved accuracy when compared to existing methods (replace number\%) via knowledge distillation from the foundation models.}}

    \item Finally, our framework gives the clients a choice of using locally stored foundation models, and allow clients to benefit from their large pretrained models (and scale of compute available) without sacrificing the model privacy or exposing their own foundation models to the federated training system. There is no restrictions on the type of foundation models.
    
    % By distilling knowledge from foundation models, we overcome the drop in overall performance observed. 
    
    
    % We when using dp-SGD {\color{red}cite}, an optimization scheme with privacy guarantees.
    % model privacy & data security
    % \item Finally, our framework allows for the flexibility in the choice of locally stored foundation models, which allows clients to benefit from their choice of foundation models and scale of computation resources, without sacrificing the privacy of their models.
\end{itemize}







\iffalse
% Paragraph: Setup + Core problem
% Setup
Federated learning (FL) is a popular training paradigm in large-scale machine learning~\cite{mcmahan2017communication} that addresses cooperative learning across distributed clients, akin to real-world settings, while preserving the privacy of data stored within them.
A typical FL framework consists of a central server that coordinates the training of a shared model by periodically aggregating local models from multiple clients, each of which are only trained using the data stored locally on the client.
% Core Problem
In practice, clients impose strict limitations on inference speeds and communications bandwidth, due to their deployment in real-world contexts, which in turn restricts them to using small-scale models.
When coupled with heterogeneous data distributions ~\cite{karimireddy2020scaffold, li2020federated} and data confidentiality restrictions, these issues present significant challenges to the overall achievable performance and robustness.

% Foundation Models: A Potential Solution
Foundation models~\cite{bommasani2021opportunities} present a potential solution to addressing poor performance under heterogeneous data distributions, with known benefits of transferable representations across a broad range of downstream tasks~\cite{radford2021learning,wang2022image}, and strong robustness to distribution shifts~\cite{ma2021simple}. Multiple recent methods explore fine-tuning transformer-based architectures and foundation models under federated settings.
% Roadblocks
However, \cite{chen2022fedtune} have shown that under extreme non-IID conditions, federated training of foundation models forces a performance worse than purely local training.
In addition, existing methods do not discuss the relatively large increase in inference time when switching to foundation models instead of small-scale alternatives like EfficientNet~\cite{tan2019efficientnet}, MobileNet~\cite{sandler2018mobilenetv2}, etc.
Further, most federated training algorithms assume the exchange of a complete set or partial subset of weights with the server, which does not comply with the privacy constraint since it has been previously shown that by capturing gradient updates or weights, a malicious user can infer multiple properties of the original data distribution~\cite{melis2019exploiting,geiping2020inverting} and in turn use this information in an adversarial manner.

% Our solution
Keeping in mind the considerations of heterogeneous data distributions, inference speed, and privacy, we propose a novel federated training framework that improves the overall performance of a small-scale model by distilling information from locally stored foundation models in clients.
% Performance under non-IID and privacy benefits
Our framework allows clients flexibility in the number and type of foundation models stored within each client, which allows the small-scale model to reap the benefits of improved performance and robustness to non-IID distributions and privacy-based optimization schemes, both of which are known to decrease overall performance.
% Size and speed benefits
In addition, our framework removes the computational burden of running a large foundation model during inference time by relying on the small-scale model to measure the overall performance of the client.
By treating the foundation model as a local model, the small-scale model as a proxy that can be shared and training them with privacy guaranteed optimization techniques like \cite{abadi2016deep,esipova2022disparate}, we ensure that data privacy is maintained.



Overall our main contributions are: 
\begin{itemize}
    \item To the best of our knowledge, we are the first to leverage foundation models in federated learning settings under a restricted computational budget. Our federated training framework increases the upper limit in performance and robustness achievable in small-scale client models under strict non-IID data settings.
    \item By distilling knowledge from foundation models, we overcome the drop in overall performance observed when using optimization schemes with privacy guarantees.
    \item Finally, our framework allows for the flexibility in the choice of locally stored foundation models, which allows clients to benefit from their choice of foundation models and scale of computation resources, without sacrificing the privacy of their models or inference speeds.
\end{itemize}
\fi

% we consider solving a federated learning problem, defined as 
% \begin{align} \label{eq:1}
% \min _{x \in \mathbb{R}^{d}}f(x):=\frac{1}{N} \sum_{i=1}^{N} f_{i}(x)
% \end{align}
% where $x \in \mathbb{R}^{d}$ denotes the model parameter and $N$ indicates the number of worker nodes. $f_{i}(x)$ is the loss function of the $i^{th}$ worker node, $\mathcal{D}_{i}$ denotes the data distribution on the $i^{th}$ worker node. $\mathcal{D}_{i}$ and $\mathcal{D}_{j}$ are different ($i \neq j$ )

% Problem setup: {\color{red}{
% The practical advancement of federated learning faces significant challenges in the form of data heterogeneity and constraints on computational resources.
% Data distribution in different clients is usually not identical, which
% referred to as the heterogeneous data setting. Often, clients are deployed to solve problems in real-world contexts which constrains their infrastructure to limited compute resources, run-time, memory, etc. With this in mind, clients are not suited to store and run state-of-the-art models, which are often extremely large in size. Thus, clients are restricted to using small-scale models which limits the maximum possible performance that can be achieved. With such accommodations, the overall system can experience reduced performance and robustness, especially when confronted with issues like serious data heterogeneity and distribution shifts that are common across federated learning. \cite{karimireddy2020scaffold, li2020federated}...
% }}\\

% Foundation Models in Federated Learning: {\color{red}{Foundation models have presented powerful zero-shot performance\cite{radford2021learning}, and knowledge transfer performance on a broad range of down-stream tasks \cite{wang2022image}. They are also shown to be effective in handle extreme heterogenous data partitions/distribution shifts, with multiple novel methods exploring the training of transformer-based architectures and foundation models under federated settings. However, they either assume the exchange of the complete or subset of weights that comprises each of these models. This assumption does not fully comply with the notion of clients being edge devices deployed in the real-world, with strong limitations in computational resources. Cite papers....

% In addition, works like FedTune have shown that under extreme non-IID settings federated training of foundation models can force worse performance than purely local training. Keeping these two considerations in mind, we propose a novel strategy that aims to improve the performance of small-scale client models by distilling information from a foundation model stored at the server. This scenario removes the computational burden of running large foundation models from the clients while improving the upper limit on both performance and robustness of small-scale client models. The proposed framework is capable of solving the issues in the FL. In this paper, we investigate }}\\

% Main contributions: {\color{red}
% \begin{itemize}
%     \item We take the first step towards leveraging the foundation models into federated learning under the restricted computational resources to propose a framework to improve inference efficiency.
%     \item With the knowledge transferred from foundation models, small-scale models in FL frameworks could correct the bias arise from data heterogeneity. 
%     \item We only communicate the model parameters of tiny models. In this case, clients could choose the personalized foundation models based on capabilities and foundation models parameters are also protected.  
% \end{itemize}
% }

% Foundation Models in Federated Learning: {\color{red}{Recently, foundation models have presented powerful zero-shot performance\cite{radford2021learning}, and knowledge transfer performance on a broad range of down-stream tasks \cite{wang2022image}. Motivated by the success of large-scale pre-trained models in centralized setting, researchers apply foundation models into FL to
% harness their exceptional transfer learning potential. Some works show foundation models are effective in handling extreme heterogenous data partitions/distribution shifts, with multiple novel methods exploring the training of transformer-based architectures and foundation models under federated settings. However, they either assume the exchange of the complete or subset of weights that comprise each of these models. This assumption does not fully comply with the notion of clients being edge devices deployed in the real-world, with strong limitations in computational resources. 

% In addition, works like FedTune have shown that under extreme non-IID settings federated training of foundation models can force worse performance than purely local training. Although foundation models could alleviate the issue of data heterogeneity, it put heavy burden on the training and inference phase. 
% Enhancing the efficiency of model inference is crucial for deploying deep learning applications on mobile devices.

% Keeping these two considerations in mind, we propose a novel strategy that aims to improve the performance of small-scale client models by distilling information from a foundation model stored at the server. This scenario removes the computational burden of running large foundation models from the clients while improving the upper limit on both performance and robustness of small-scale client models. The proposed framework is capable of solving the issues in the FL. In this paper, we investigate }}\\

% Main contributions: {\color{red}
% \begin{itemize}
%     \item We take the first step towards leveraging the foundation models into federated learning under restricted computational resources. We propose a  lightweight FL framework to improve inference efficiency. It helps the deploy of tiny models from federated learning on edge devices. 
%     \item We only communicate the model parameters of tiny models. In this case, clients could choose the personalized foundation models based on capabilities and foundation models parameters are also protected.  
%     \item With the instruction of knowledge transferred from foundation models, tiny models in *** frameworks could correct the bias during the training arising from data heterogeneity and performance is increased largely. Experiments on a variety of settings show the remarkable advantages of *** .
% \end{itemize}
% }

==> tex/related_work.tex <==
\section{Related Work}
\label{sec:related_work}
\paragraph{Federated Learning} Federated learning is a distributed machine learning paradigm that enables multiple clients to collaboratively train a shared model while keeping their data private.
% local, thereby preserving data privacy. 
\cite{mcmahan2017communication} proposed FedAvg as an effective solution to collaboratively train a global model by using periodic model averaging. 
Since then, federated learning has been adopted across a range of application domains including computer vision~\cite{li2021survey}, natural language processing~\cite{liu2021federated}, speech recognition~\cite{guliani2021training}, health care~\cite{xu2021federated}, Internet of Things~\cite{ramaswamy2019federated}, and many others, to successfully leverage knowledge distributed across multiple devices.
More recently, there has been a concerted effort in tackling key challenges of federated learning such as, performance under heterogeneous data settings~\cite{woodworth2020local, khaled2020tighter} , reduced communication efficiency~\cite{rothchild2020fetchsgd,haddadpour2021federated}, improved privacy~\cite{geyer2017differentially,wei2020federated}, etc.~\cite{karimireddy2020scaffold,li2020federated,reddi2020adaptive}. 

\paragraph{Heterogenous Data Distributions}
Frequently, client data can have non identical distributions which cause large drops in accuracy during federated training. 
In these cases, naive aggregation methods such as FedAvg cannot guarantee model convergence to a local minimum \cite{zhao2018federated, li2020federated, hsieh2020non,li2020federated1}. 
To tackle this challenge, personalized FL-algorithms such as FedProx~\cite{li2020federated1} add a proximal term to local training objectives to protect models in each client from over-fitting to the local data distribution; other approaches such as regularization~\cite{t2020personalized}, model mixture~\cite{deng2020adaptive, mansour2020three, hanzely2020federated}, and clustered clients \cite{sattler2020clustered, cho2021personalized} have been introduced to stabilize the performance of client's models. 
An alternative set of works use multi-task learning~\cite{smith2017federated}, which trains on different tasks simultaneously, and meta-learning~\cite{fallah2020personalized}, which rapidly adapts the global model to each client's local data distribution, to help alleviate the impact of skewed data distributions.
In this work, we tackle the issue of heterogeneous data distributions through the use of foundation models, which have been shown mitigate this issue without the need for additional data.


\paragraph{Foundation Models} The past few years have witnessed the rapid development of foundation models with a notable trend towards the integration of language~\cite{radford2018improving, devlin2018bert,radford2021learning}, vision~\cite{bao2021beit}, and audio modalities~\cite{tang2023any}. 
Leveraging the power of pre-training on large-scale datasets, we can seamlessly apply these models to a wide range of tasks. 
Motivated by the success of foundation models in FL, be it in improving the robustness of clients to distribution shifts and heterogeneous data distributions~\cite{qu2022rethinking}, or improving the overall performance of the system~\cite{chen2022fedtune, guo2023promptfl, zhao2023fedprompt, lu2023fedclip, guo2023pfedprompt}, there have been a number of recent works that study the impact of different foundation model fine-tuning approaches in the FL setting.
Although foundation models strongly benefit performance under heterogeneous data settings, directly training and evaluating on foundation models increases the computational burden on the client and increases their latency during inference. 
This hinders their deployment in real-world settings.
Instead, our framework leverages the benefits of foundation models, stored locally, to help improve the performance and robustness of small-scale models, which have significantly lower communication and inference overheads.

\paragraph{Inference Efficiency}
Of particular interest to us are FL strategies that tackle the problem of maintaining efficiency during inference. 
For example, \cite{xu2019elfish} employ dropout to minimize latency during inference, while \cite{jiang2022model} propose a method to adaptively prune parameters during federated training so that the final model matches a client's on-device constraints, with \cite{zhou2022federated} providing theoretical analysis on the convergence of such algorithms. 
\cite{li2021fedmask} introduce federated learning with personalized and structured sparse masks and HetroFL~\cite{li2021hermes} suggest the creation of diverse local models as sub-networks of the global model by selecting key continuous parameters, in a layer by layer fashion through structured pruning. 
An important distinction between existing works that address inference efficiency and our approach is their use of pruning as a platform to personalize and match the communication and inference restrictions in each client.
In this work, our focus is on fixing the available communication and inference budgets and improving the upper limit on performance from client model's that satisfy those conditions.
These two approaches are complementary and can be combined to further magnify their impact.

\paragraph{Privacy}
To mitigate data privacy concerns in FL, \cite{shen2020federated} introduce an FL framework which allows clients to train both a meme/proxy model and a private model using mutual learning~\cite{zhang2018deep}. 
Only the meme/proxy model is shared with server, thus reducing the risk of data exposure. 
However, \cite{melis2019exploiting} and \cite{geiping2020inverting} highlight the vulnerabilities associated with the capture of model weights/updates during the exchange of information between clients and the server.
This includes the inference of class prototypes, key properties and in certain cases the recreation of input images from the training data.
To provide privacy guarantees, one can use methods like differential privacy \cite{wei2020federated, zhao2020local, seif2020wireless, papernot2018scalable, abadi2016deep, dwork2010boosting, dwork2009differential}, secure multiparty computation \cite{pettai2015combining}, secret sharing \cite{bonawitz2017practical}, homomorphic encryption and hybrid methods \cite{xu2019hybridalpha, truex2019hybrid, pettai2015combining}.
With this in mind, ProxyFL~\cite{kalra2023decentralized} proposes a formulation similar to \cite{shen2020federated} where clients maintain a private and a proxy model that are trained using mutual learning.
However, in ProxyFL each client uses DP-SGD~\cite{abadi2016deep} during training, which provides measurable guarantees~\cite{balle2020hypothesis} for differential privacy. 
In a similar fashion, \cite{wei2020federated} propose an FL framework based on differential privacy (DP) by adding artificial noise to parameters during local training in the clients to obfuscate and protect information about client data distributions.
A key drawback of existing algorithms which guarantee differential privacy is the drop in performance of the global model relative to algorithms that do not account for it.
Inspired by methods that actively tackle privacy concerns, we adopt the use of DP-SGD and study the impact of distilling from foundation models, which are known to have a high performance ceiling on image classification tasks.

\paragraph{Distillation}
Knowledge distillation is a teaching technique that can transfer valuable insights and generalization capabilities from a teacher model to a student model~\cite{hinton2015distilling,anil2018large, zhang2018deep, zhang2021adversarial}. 
% There are numerous works that study knowledge distillation based on the choice of dataset~\cite{wang2018dataset}, core-data selection~\cite{sener2017active} and  reconstructed data~\cite{yoo2019knowledge, micaelli2019zero}.
Within the domain of FL, \cite{lin2020ensemble} explore adaptable aggregation methods with ensemble distillation to obtain the global model in the server, while \cite{sattler2021fedaux} use an auxiliary dataset to weight and ensemble local models from each client.
\cite{seo202216} introduce FedDistill, a method that extracts statistics related to the logit-vector from different client models, which are then shared with the remaining clients to facilitate knowledge distillation. 
\cite{zhu2021data} present a data-free knowledge distillation approach (FEDGEN) to address data heterogeneity in FL, where at the server they train a generative model by combining information from clients to train a generator, which is then used to train client models. 
\cite{cho2021personalized} propose a co-distillation based personalized federated learning method to allow cross-architecture training.
In our approach, we study the impact of knowledge distillation~\cite{hinton2015distilling} on the performance of small-scale client models without the use of excessive data, augmentations or model sharing so as to maintain privacy and provide guidance with respect to how can foundation models be effectively used in federated learning. 
